ReFoCUS: Reinforcement-guided Frame Optimization for Contextual Understanding

Recent progress in Large Multi-modal Models (LMMs) has enabled effective vision-language reasoning, yet the ability to video understanding remains constrained by suboptimal frame selection strategies, albeit with the rapid development of video-specialized LMMs. Prior works attempted to solve this with static heuristics or external retrieval modules to feed frame-level information, but these approaches often fail to capture visual cues grounded to the given user queries conflating raw visual dynamics with true semantic relevance. In this paper, we introduce ReFoCUS (Reinforcement-guided Frame Optimization for Contextual UnderStanding), the first framework to integrate online policy-gradient reinforcement learning into frame-level optimization for video-LLMs. ReFoCUS aims to learn a frame selection policy, leveraging reward signals derived from reference models to capture their underlying scoring behavior over frame combinations that best support temporally grounded responses. To efficiently explore the large combinatorial frame space, we employ an autoregressive and query-conditional selection architecture that ensures contextual consistency while reducing complexity. Our policy learning removes the need for explicit frame-level supervision, as it implicitly discovers optimal and semantically consistent frame compositions. ReFoCUS consistently improves reasoning accuracy across multiple video QA benchmarks, demonstrating the advantage of aligning frame selection with model-internal utility.

==> assets/039-1/MDP3/response.tex <==
\WA{B. 03:00.}

==> assets/039-1/MDP3/time1.tex <==
0:00

==> assets/039-1/MDP3/time10.tex <==
0:24

==> assets/039-1/MDP3/time11.tex <==
0:25

==> assets/039-1/MDP3/time12.tex <==
0:27

==> assets/039-1/MDP3/time13.tex <==
0:28

==> assets/039-1/MDP3/time14.tex <==
0:30

==> assets/039-1/MDP3/time15.tex <==
0:37

==> assets/039-1/MDP3/time16.tex <==
0:40

==> assets/039-1/MDP3/time17.tex <==
0:41

==> assets/039-1/MDP3/time18.tex <==
0:43

==> assets/039-1/MDP3/time19.tex <==
0:46

==> assets/039-1/MDP3/time2.tex <==
0:06

==> assets/039-1/MDP3/time20.tex <==
0:49

==> assets/039-1/MDP3/time21.tex <==
1:00

==> assets/039-1/MDP3/time22.tex <==
1:05

==> assets/039-1/MDP3/time23.tex <==
1:06

==> assets/039-1/MDP3/time24.tex <==
1:08

==> assets/039-1/MDP3/time25.tex <==
1:11

==> assets/039-1/MDP3/time26.tex <==
1:16

==> assets/039-1/MDP3/time27.tex <==
1:19

==> assets/039-1/MDP3/time28.tex <==
1:20

==> assets/039-1/MDP3/time29.tex <==
1:21

==> assets/039-1/MDP3/time3.tex <==
0:09

==> assets/039-1/MDP3/time30.tex <==
1:38

==> assets/039-1/MDP3/time31.tex <==
1:41

==> assets/039-1/MDP3/time32.tex <==
1:51

==> assets/039-1/MDP3/time4.tex <==
0:10

==> assets/039-1/MDP3/time5.tex <==
0:15

==> assets/039-1/MDP3/time6.tex <==
0:18

==> assets/039-1/MDP3/time7.tex <==
0:20

==> assets/039-1/MDP3/time8.tex <==
0:21

==> assets/039-1/MDP3/time9.tex <==
0:23

==> assets/039-1/ReFoCUS/response.tex <==
\ANS{D. 05:00.}

==> assets/039-1/ReFoCUS/time1.tex <==
0:23

==> assets/039-1/ReFoCUS/time10.tex <==
0:31

==> assets/039-1/ReFoCUS/time11.tex <==
0:31

==> assets/039-1/ReFoCUS/time12.tex <==
0:32

==> assets/039-1/ReFoCUS/time13.tex <==
0:32

==> assets/039-1/ReFoCUS/time14.tex <==
0:33

==> assets/039-1/ReFoCUS/time15.tex <==
0:33

==> assets/039-1/ReFoCUS/time16.tex <==
0:33

==> assets/039-1/ReFoCUS/time17.tex <==
0:33

==> assets/039-1/ReFoCUS/time18.tex <==
0:34

==> assets/039-1/ReFoCUS/time19.tex <==
0:34

==> assets/039-1/ReFoCUS/time2.tex <==
0:23

==> assets/039-1/ReFoCUS/time20.tex <==
0:34

==> assets/039-1/ReFoCUS/time21.tex <==
0:34

==> assets/039-1/ReFoCUS/time22.tex <==
0:35

==> assets/039-1/ReFoCUS/time23.tex <==
0:36

==> assets/039-1/ReFoCUS/time24.tex <==
0:36

==> assets/039-1/ReFoCUS/time25.tex <==
0:42

==> assets/039-1/ReFoCUS/time26.tex <==
0:42

==> assets/039-1/ReFoCUS/time27.tex <==
0:43

==> assets/039-1/ReFoCUS/time28.tex <==
0:43

==> assets/039-1/ReFoCUS/time29.tex <==
0:43

==> assets/039-1/ReFoCUS/time3.tex <==
0:23

==> assets/039-1/ReFoCUS/time30.tex <==
0:44

==> assets/039-1/ReFoCUS/time31.tex <==
0:49

==> assets/039-1/ReFoCUS/time32.tex <==
0:50

==> assets/039-1/ReFoCUS/time4.tex <==
0:24

==> assets/039-1/ReFoCUS/time5.tex <==
0:30

==> assets/039-1/ReFoCUS/time6.tex <==
0:30

==> assets/039-1/ReFoCUS/time7.tex <==
0:30

==> assets/039-1/ReFoCUS/time8.tex <==
0:30

==> assets/039-1/ReFoCUS/time9.tex <==
0:31

==> assets/039-1/Uniform/response.tex <==
\WA{C. 11:00.}

==> assets/039-1/Uniform/time1.tex <==
0:00

==> assets/039-1/Uniform/time10.tex <==
0:32

==> assets/039-1/Uniform/time11.tex <==
0:36

==> assets/039-1/Uniform/time12.tex <==
0:39

==> assets/039-1/Uniform/time13.tex <==
0:43

==> assets/039-1/Uniform/time14.tex <==
0:46

==> assets/039-1/Uniform/time15.tex <==
0:50

==> assets/039-1/Uniform/time16.tex <==
0:54

==> assets/039-1/Uniform/time17.tex <==
0:57

==> assets/039-1/Uniform/time18.tex <==
1:01

==> assets/039-1/Uniform/time19.tex <==
1:04

==> assets/039-1/Uniform/time2.tex <==
0:03

==> assets/039-1/Uniform/time20.tex <==
1:08

==> assets/039-1/Uniform/time21.tex <==
1:12

==> assets/039-1/Uniform/time22.tex <==
1:15

==> assets/039-1/Uniform/time23.tex <==
1:19

==> assets/039-1/Uniform/time24.tex <==
1:22

==> assets/039-1/Uniform/time25.tex <==
1:26

==> assets/039-1/Uniform/time26.tex <==
1:30

==> assets/039-1/Uniform/time27.tex <==
1:33

==> assets/039-1/Uniform/time28.tex <==
1:37

==> assets/039-1/Uniform/time29.tex <==
1:40

==> assets/039-1/Uniform/time3.tex <==
0:07

==> assets/039-1/Uniform/time30.tex <==
1:44

==> assets/039-1/Uniform/time31.tex <==
1:48

==> assets/039-1/Uniform/time32.tex <==
1:51

==> assets/039-1/Uniform/time4.tex <==
0:10

==> assets/039-1/Uniform/time5.tex <==
0:14

==> assets/039-1/Uniform/time6.tex <==
0:17

==> assets/039-1/Uniform/time7.tex <==
0:21

==> assets/039-1/Uniform/time8.tex <==
0:25

==> assets/039-1/Uniform/time9.tex <==
0:28

==> assets/039-1/options.tex <==
\item A. 08:00.
\item B. 03:00.
\item C. 11:00.
\ANS{\item D. 05:00.}


==> assets/039-1/questions.tex <==
Which time is displayed on the clock in the video?

==> assets/041-2/MDP3/response.tex <==
\WA{A. 2.}

==> assets/041-2/MDP3/time1.tex <==
0:00

==> assets/041-2/MDP3/time10.tex <==
0:16

==> assets/041-2/MDP3/time11.tex <==
0:20

==> assets/041-2/MDP3/time12.tex <==
0:21

==> assets/041-2/MDP3/time13.tex <==
0:23

==> assets/041-2/MDP3/time14.tex <==
0:25

==> assets/041-2/MDP3/time15.tex <==
0:26

==> assets/041-2/MDP3/time16.tex <==
0:29

==> assets/041-2/MDP3/time17.tex <==
0:30

==> assets/041-2/MDP3/time18.tex <==
0:31

==> assets/041-2/MDP3/time19.tex <==
0:35

==> assets/041-2/MDP3/time2.tex <==
0:01

==> assets/041-2/MDP3/time20.tex <==
0:35

==> assets/041-2/MDP3/time21.tex <==
0:39

==> assets/041-2/MDP3/time22.tex <==
0:40

==> assets/041-2/MDP3/time23.tex <==
0:42

==> assets/041-2/MDP3/time24.tex <==
0:44

==> assets/041-2/MDP3/time25.tex <==
0:46

==> assets/041-2/MDP3/time26.tex <==
0:49

==> assets/041-2/MDP3/time27.tex <==
0:54

==> assets/041-2/MDP3/time28.tex <==
0:56

==> assets/041-2/MDP3/time29.tex <==
0:59

==> assets/041-2/MDP3/time3.tex <==
0:03

==> assets/041-2/MDP3/time30.tex <==
1:00

==> assets/041-2/MDP3/time31.tex <==
1:05

==> assets/041-2/MDP3/time32.tex <==
1:08

==> assets/041-2/MDP3/time4.tex <==
0:03

==> assets/041-2/MDP3/time5.tex <==
0:05

==> assets/041-2/MDP3/time6.tex <==
0:06

==> assets/041-2/MDP3/time7.tex <==
0:06

==> assets/041-2/MDP3/time8.tex <==
0:12

==> assets/041-2/MDP3/time9.tex <==
0:13

==> assets/041-2/ReFoCUS/response.tex <==
\WA{C. 3.}

==> assets/041-2/ReFoCUS/time1.tex <==
0:03

==> assets/041-2/ReFoCUS/time10.tex <==
0:08

==> assets/041-2/ReFoCUS/time11.tex <==
0:08

==> assets/041-2/ReFoCUS/time12.tex <==
0:08

==> assets/041-2/ReFoCUS/time13.tex <==
0:10

==> assets/041-2/ReFoCUS/time14.tex <==
0:12

==> assets/041-2/ReFoCUS/time15.tex <==
0:13

==> assets/041-2/ReFoCUS/time16.tex <==
0:16

==> assets/041-2/ReFoCUS/time17.tex <==
0:16

==> assets/041-2/ReFoCUS/time18.tex <==
0:16

==> assets/041-2/ReFoCUS/time19.tex <==
0:16

==> assets/041-2/ReFoCUS/time2.tex <==
0:05

==> assets/041-2/ReFoCUS/time20.tex <==
0:17

==> assets/041-2/ReFoCUS/time21.tex <==
0:17

==> assets/041-2/ReFoCUS/time22.tex <==
0:17

==> assets/041-2/ReFoCUS/time23.tex <==
0:17

==> assets/041-2/ReFoCUS/time24.tex <==
0:18

==> assets/041-2/ReFoCUS/time25.tex <==
0:19

==> assets/041-2/ReFoCUS/time26.tex <==
0:19

==> assets/041-2/ReFoCUS/time27.tex <==
0:19

==> assets/041-2/ReFoCUS/time28.tex <==
0:20

==> assets/041-2/ReFoCUS/time29.tex <==
0:20

==> assets/041-2/ReFoCUS/time3.tex <==
0:05

==> assets/041-2/ReFoCUS/time30.tex <==
0:20

==> assets/041-2/ReFoCUS/time31.tex <==
0:20

==> assets/041-2/ReFoCUS/time32.tex <==
0:21

==> assets/041-2/ReFoCUS/time4.tex <==
0:06

==> assets/041-2/ReFoCUS/time5.tex <==
0:06

==> assets/041-2/ReFoCUS/time6.tex <==
0:07

==> assets/041-2/ReFoCUS/time7.tex <==
0:07

==> assets/041-2/ReFoCUS/time8.tex <==
0:07

==> assets/041-2/ReFoCUS/time9.tex <==
0:07

==> assets/041-2/Uniform/response.tex <==
\WA{C. 3.}

==> assets/041-2/Uniform/time1.tex <==
0:00

==> assets/041-2/Uniform/time10.tex <==
0:20

==> assets/041-2/Uniform/time11.tex <==
0:22

==> assets/041-2/Uniform/time12.tex <==
0:25

==> assets/041-2/Uniform/time13.tex <==
0:27

==> assets/041-2/Uniform/time14.tex <==
0:29

==> assets/041-2/Uniform/time15.tex <==
0:32

==> assets/041-2/Uniform/time16.tex <==
0:34

==> assets/041-2/Uniform/time17.tex <==
0:36

==> assets/041-2/Uniform/time18.tex <==
0:38

==> assets/041-2/Uniform/time19.tex <==
0:41

==> assets/041-2/Uniform/time2.tex <==
0:02

==> assets/041-2/Uniform/time20.tex <==
0:43

==> assets/041-2/Uniform/time21.tex <==
0:45

==> assets/041-2/Uniform/time22.tex <==
0:48

==> assets/041-2/Uniform/time23.tex <==
0:50

==> assets/041-2/Uniform/time24.tex <==
0:52

==> assets/041-2/Uniform/time25.tex <==
0:54

==> assets/041-2/Uniform/time26.tex <==
0:57

==> assets/041-2/Uniform/time27.tex <==
0:59

==> assets/041-2/Uniform/time28.tex <==
1:01

==> assets/041-2/Uniform/time29.tex <==
1:04

==> assets/041-2/Uniform/time3.tex <==
0:04

==> assets/041-2/Uniform/time30.tex <==
1:06

==> assets/041-2/Uniform/time31.tex <==
1:08

==> assets/041-2/Uniform/time32.tex <==
1:10

==> assets/041-2/Uniform/time4.tex <==
0:06

==> assets/041-2/Uniform/time5.tex <==
0:09

==> assets/041-2/Uniform/time6.tex <==
0:11

==> assets/041-2/Uniform/time7.tex <==
0:13

==> assets/041-2/Uniform/time8.tex <==
0:16

==> assets/041-2/Uniform/time9.tex <==
0:18

==> assets/041-2/options.tex <==
\item A. 2.
\ANS{\item B. 4.}
\item C. 3.
\item D. 1.


==> assets/041-2/questions.tex <==
How many times is the sun visible in the video?

==> assets/206-1/MDP3/response.tex <==
\WA{B. 6.}

==> assets/206-1/MDP3/time1.tex <==
0:00

==> assets/206-1/MDP3/time10.tex <==
0:20

==> assets/206-1/MDP3/time11.tex <==
0:23

==> assets/206-1/MDP3/time12.tex <==
0:24

==> assets/206-1/MDP3/time13.tex <==
0:29

==> assets/206-1/MDP3/time14.tex <==
0:33

==> assets/206-1/MDP3/time15.tex <==
0:35

==> assets/206-1/MDP3/time16.tex <==
0:40

==> assets/206-1/MDP3/time17.tex <==
0:42

==> assets/206-1/MDP3/time18.tex <==
0:47

==> assets/206-1/MDP3/time19.tex <==
0:53

==> assets/206-1/MDP3/time2.tex <==
0:07

==> assets/206-1/MDP3/time20.tex <==
0:59

==> assets/206-1/MDP3/time21.tex <==
1:00

==> assets/206-1/MDP3/time22.tex <==
1:00

==> assets/206-1/MDP3/time23.tex <==
1:03

==> assets/206-1/MDP3/time24.tex <==
1:04

==> assets/206-1/MDP3/time25.tex <==
1:05

==> assets/206-1/MDP3/time26.tex <==
1:07

==> assets/206-1/MDP3/time27.tex <==
1:08

==> assets/206-1/MDP3/time28.tex <==
1:09

==> assets/206-1/MDP3/time29.tex <==
1:09

==> assets/206-1/MDP3/time3.tex <==
0:10

==> assets/206-1/MDP3/time30.tex <==
1:10

==> assets/206-1/MDP3/time31.tex <==
1:11

==> assets/206-1/MDP3/time32.tex <==
1:12

==> assets/206-1/MDP3/time4.tex <==
0:10

==> assets/206-1/MDP3/time5.tex <==
0:12

==> assets/206-1/MDP3/time6.tex <==
0:14

==> assets/206-1/MDP3/time7.tex <==
0:14

==> assets/206-1/MDP3/time8.tex <==
0:16

==> assets/206-1/MDP3/time9.tex <==
0:18

==> assets/206-1/ReFoCUS/response.tex <==
\ANS{A. 7.}

==> assets/206-1/ReFoCUS/time1.tex <==
0:22

==> assets/206-1/ReFoCUS/time10.tex <==
0:49

==> assets/206-1/ReFoCUS/time11.tex <==
0:50

==> assets/206-1/ReFoCUS/time12.tex <==
0:50

==> assets/206-1/ReFoCUS/time13.tex <==
0:50

==> assets/206-1/ReFoCUS/time14.tex <==
0:50

==> assets/206-1/ReFoCUS/time15.tex <==
0:51

==> assets/206-1/ReFoCUS/time16.tex <==
0:51

==> assets/206-1/ReFoCUS/time17.tex <==
0:52

==> assets/206-1/ReFoCUS/time18.tex <==
0:52

==> assets/206-1/ReFoCUS/time19.tex <==
0:53

==> assets/206-1/ReFoCUS/time2.tex <==
0:47

==> assets/206-1/ReFoCUS/time20.tex <==
0:53

==> assets/206-1/ReFoCUS/time21.tex <==
0:54

==> assets/206-1/ReFoCUS/time22.tex <==
0:54

==> assets/206-1/ReFoCUS/time23.tex <==
0:54

==> assets/206-1/ReFoCUS/time24.tex <==
0:55

==> assets/206-1/ReFoCUS/time25.tex <==
0:55

==> assets/206-1/ReFoCUS/time26.tex <==
0:56

==> assets/206-1/ReFoCUS/time27.tex <==
0:56

==> assets/206-1/ReFoCUS/time28.tex <==
0:57

==> assets/206-1/ReFoCUS/time29.tex <==
0:57

==> assets/206-1/ReFoCUS/time3.tex <==
0:48

==> assets/206-1/ReFoCUS/time30.tex <==
0:58

==> assets/206-1/ReFoCUS/time31.tex <==
0:58

==> assets/206-1/ReFoCUS/time32.tex <==
0:58

==> assets/206-1/ReFoCUS/time4.tex <==
0:48

==> assets/206-1/ReFoCUS/time5.tex <==
0:48

==> assets/206-1/ReFoCUS/time6.tex <==
0:48

==> assets/206-1/ReFoCUS/time7.tex <==
0:49

==> assets/206-1/ReFoCUS/time8.tex <==
0:49

==> assets/206-1/ReFoCUS/time9.tex <==
0:49

==> assets/206-1/Uniform/response.tex <==
\WA{B. 6.}

==> assets/206-1/Uniform/time1.tex <==
0:00

==> assets/206-1/Uniform/time10.tex <==
0:21

==> assets/206-1/Uniform/time11.tex <==
0:23

==> assets/206-1/Uniform/time12.tex <==
0:25

==> assets/206-1/Uniform/time13.tex <==
0:28

==> assets/206-1/Uniform/time14.tex <==
0:30

==> assets/206-1/Uniform/time15.tex <==
0:32

==> assets/206-1/Uniform/time16.tex <==
0:35

==> assets/206-1/Uniform/time17.tex <==
0:37

==> assets/206-1/Uniform/time18.tex <==
0:39

==> assets/206-1/Uniform/time19.tex <==
0:42

==> assets/206-1/Uniform/time2.tex <==
0:02

==> assets/206-1/Uniform/time20.tex <==
0:44

==> assets/206-1/Uniform/time21.tex <==
0:46

==> assets/206-1/Uniform/time22.tex <==
0:49

==> assets/206-1/Uniform/time23.tex <==
0:51

==> assets/206-1/Uniform/time24.tex <==
0:53

==> assets/206-1/Uniform/time25.tex <==
0:56

==> assets/206-1/Uniform/time26.tex <==
0:58

==> assets/206-1/Uniform/time27.tex <==
1:00

==> assets/206-1/Uniform/time28.tex <==
1:03

==> assets/206-1/Uniform/time29.tex <==
1:05

==> assets/206-1/Uniform/time3.tex <==
0:04

==> assets/206-1/Uniform/time30.tex <==
1:08

==> assets/206-1/Uniform/time31.tex <==
1:10

==> assets/206-1/Uniform/time32.tex <==
1:12

==> assets/206-1/Uniform/time4.tex <==
0:07

==> assets/206-1/Uniform/time5.tex <==
0:09

==> assets/206-1/Uniform/time6.tex <==
0:11

==> assets/206-1/Uniform/time7.tex <==
0:14

==> assets/206-1/Uniform/time8.tex <==
0:16

==> assets/206-1/Uniform/time9.tex <==
0:18

==> assets/206-1/options.tex <==
\item \ANS{A. 7.}
\item B. 6.
\item C. 5.
\item D. 8.


==> assets/206-1/questions.tex <==
What is the total number of people in the video?

==> assets/345-1/MDP3/response.tex <==
\WA{B. 50 days.}

==> assets/345-1/MDP3/time1.tex <==
0:10

==> assets/345-1/MDP3/time10.tex <==
2:22

==> assets/345-1/MDP3/time11.tex <==
2:32

==> assets/345-1/MDP3/time12.tex <==
2:43

==> assets/345-1/MDP3/time13.tex <==
3:09

==> assets/345-1/MDP3/time14.tex <==
3:14

==> assets/345-1/MDP3/time15.tex <==
3:25

==> assets/345-1/MDP3/time16.tex <==
3:41

==> assets/345-1/MDP3/time17.tex <==
3:51

==> assets/345-1/MDP3/time18.tex <==
4:02

==> assets/345-1/MDP3/time19.tex <==
4:07

==> assets/345-1/MDP3/time2.tex <==
0:15

==> assets/345-1/MDP3/time20.tex <==
4:23

==> assets/345-1/MDP3/time21.tex <==
4:33

==> assets/345-1/MDP3/time22.tex <==
4:55

==> assets/345-1/MDP3/time23.tex <==
5:00

==> assets/345-1/MDP3/time24.tex <==
5:10

==> assets/345-1/MDP3/time25.tex <==
5:58

==> assets/345-1/MDP3/time26.tex <==
6:19

==> assets/345-1/MDP3/time27.tex <==
6:40

==> assets/345-1/MDP3/time28.tex <==
7:48

==> assets/345-1/MDP3/time29.tex <==
9:23

==> assets/345-1/MDP3/time3.tex <==
0:36

==> assets/345-1/MDP3/time30.tex <==
10:21

==> assets/345-1/MDP3/time31.tex <==
10:32

==> assets/345-1/MDP3/time32.tex <==
10:53

==> assets/345-1/MDP3/time4.tex <==
0:42

==> assets/345-1/MDP3/time5.tex <==
0:52

==> assets/345-1/MDP3/time6.tex <==
1:08

==> assets/345-1/MDP3/time7.tex <==
1:19

==> assets/345-1/MDP3/time8.tex <==
1:34

==> assets/345-1/MDP3/time9.tex <==
2:01

==> assets/345-1/ReFoCUS/response.tex <==
\ANS{A. 160 days}

==> assets/345-1/ReFoCUS/time1.tex <==
0:36

==> assets/345-1/ReFoCUS/time10.tex <==
1:08

==> assets/345-1/ReFoCUS/time11.tex <==
1:09

==> assets/345-1/ReFoCUS/time12.tex <==
1:18

==> assets/345-1/ReFoCUS/time13.tex <==
1:21

==> assets/345-1/ReFoCUS/time14.tex <==
1:23

==> assets/345-1/ReFoCUS/time15.tex <==
1:34

==> assets/345-1/ReFoCUS/time16.tex <==
1:35

==> assets/345-1/ReFoCUS/time17.tex <==
1:36

==> assets/345-1/ReFoCUS/time18.tex <==
1:44

==> assets/345-1/ReFoCUS/time19.tex <==
1:46

==> assets/345-1/ReFoCUS/time2.tex <==
0:44

==> assets/345-1/ReFoCUS/time20.tex <==
1:48

==> assets/345-1/ReFoCUS/time21.tex <==
1:49

==> assets/345-1/ReFoCUS/time22.tex <==
2:21

==> assets/345-1/ReFoCUS/time23.tex <==
2:31

==> assets/345-1/ReFoCUS/time24.tex <==
2:33

==> assets/345-1/ReFoCUS/time25.tex <==
2:34

==> assets/345-1/ReFoCUS/time26.tex <==
3:09

==> assets/345-1/ReFoCUS/time27.tex <==
4:48

==> assets/345-1/ReFoCUS/time28.tex <==
4:50

==> assets/345-1/ReFoCUS/time29.tex <==
4:51

==> assets/345-1/ReFoCUS/time3.tex <==
0:45

==> assets/345-1/ReFoCUS/time30.tex <==
4:53

==> assets/345-1/ReFoCUS/time31.tex <==
4:54

==> assets/345-1/ReFoCUS/time32.tex <==
5:58

==> assets/345-1/ReFoCUS/time4.tex <==
0:47

==> assets/345-1/ReFoCUS/time5.tex <==
0:51

==> assets/345-1/ReFoCUS/time6.tex <==
0:52

==> assets/345-1/ReFoCUS/time7.tex <==
0:53

==> assets/345-1/ReFoCUS/time8.tex <==
0:54

==> assets/345-1/ReFoCUS/time9.tex <==
0:56

==> assets/345-1/Uniform/response.tex <==
\WA{B. 50 days.}

==> assets/345-1/Uniform/time1.tex <==
0:00

==> assets/345-1/Uniform/time10.tex <==
3:14

==> assets/345-1/Uniform/time11.tex <==
3:35

==> assets/345-1/Uniform/time12.tex <==
3:57

==> assets/345-1/Uniform/time13.tex <==
4:19

==> assets/345-1/Uniform/time14.tex <==
4:40

==> assets/345-1/Uniform/time15.tex <==
5:02

==> assets/345-1/Uniform/time16.tex <==
5:23

==> assets/345-1/Uniform/time17.tex <==
5:45

==> assets/345-1/Uniform/time18.tex <==
6:06

==> assets/345-1/Uniform/time19.tex <==
6:28

==> assets/345-1/Uniform/time2.tex <==
0:21

==> assets/345-1/Uniform/time20.tex <==
6:50

==> assets/345-1/Uniform/time21.tex <==
7:11

==> assets/345-1/Uniform/time22.tex <==
7:33

==> assets/345-1/Uniform/time23.tex <==
7:54

==> assets/345-1/Uniform/time24.tex <==
8:16

==> assets/345-1/Uniform/time25.tex <==
8:38

==> assets/345-1/Uniform/time26.tex <==
8:59

==> assets/345-1/Uniform/time27.tex <==
9:21

==> assets/345-1/Uniform/time28.tex <==
9:42

==> assets/345-1/Uniform/time29.tex <==
10:04

==> assets/345-1/Uniform/time3.tex <==
0:43

==> assets/345-1/Uniform/time30.tex <==
10:25

==> assets/345-1/Uniform/time31.tex <==
10:47

==> assets/345-1/Uniform/time32.tex <==
11:09

==> assets/345-1/Uniform/time4.tex <==
1:04

==> assets/345-1/Uniform/time5.tex <==
1:26

==> assets/345-1/Uniform/time6.tex <==
1:47

==> assets/345-1/Uniform/time7.tex <==
2:09

==> assets/345-1/Uniform/time8.tex <==
2:31

==> assets/345-1/Uniform/time9.tex <==
2:52

==> assets/345-1/options.tex <==
\item \ANS{A. 160 days.}
\item B. 50 days.
\item C. 180 days.
\item D. 19 days.


==> assets/345-1/questions.tex <==
The video shows how long it takes to drive from the Earth to the Moon?

==> assets/419-2/MDP3/response.tex <==
\WA{D. Middle of the video.}

==> assets/419-2/MDP3/time1.tex <==
0:00

==> assets/419-2/MDP3/time10.tex <==
1:33

==> assets/419-2/MDP3/time11.tex <==
1:51

==> assets/419-2/MDP3/time12.tex <==
1:57

==> assets/419-2/MDP3/time13.tex <==
2:26

==> assets/419-2/MDP3/time14.tex <==
2:38

==> assets/419-2/MDP3/time15.tex <==
2:44

==> assets/419-2/MDP3/time16.tex <==
2:50

==> assets/419-2/MDP3/time17.tex <==
4:36

==> assets/419-2/MDP3/time18.tex <==
5:11

==> assets/419-2/MDP3/time19.tex <==
5:34

==> assets/419-2/MDP3/time2.tex <==
0:11

==> assets/419-2/MDP3/time20.tex <==
5:40

==> assets/419-2/MDP3/time21.tex <==
5:58

==> assets/419-2/MDP3/time22.tex <==
6:39

==> assets/419-2/MDP3/time23.tex <==
6:45

==> assets/419-2/MDP3/time24.tex <==
7:08

==> assets/419-2/MDP3/time25.tex <==
8:54

==> assets/419-2/MDP3/time26.tex <==
9:06

==> assets/419-2/MDP3/time27.tex <==
9:18

==> assets/419-2/MDP3/time28.tex <==
9:29

==> assets/419-2/MDP3/time29.tex <==
9:41

==> assets/419-2/MDP3/time3.tex <==
0:35

==> assets/419-2/MDP3/time30.tex <==
10:40

==> assets/419-2/MDP3/time31.tex <==
11:27

==> assets/419-2/MDP3/time32.tex <==
12:14

==> assets/419-2/MDP3/time4.tex <==
0:46

==> assets/419-2/MDP3/time5.tex <==
0:52

==> assets/419-2/MDP3/time6.tex <==
0:58

==> assets/419-2/MDP3/time7.tex <==
1:04

==> assets/419-2/MDP3/time8.tex <==
1:22

==> assets/419-2/MDP3/time9.tex <==
1:28

==> assets/419-2/ReFoCUS/response.tex <==
\ANS{C. Beggining of the video}

==> assets/419-2/ReFoCUS/time1.tex <==
0:07

==> assets/419-2/ReFoCUS/time10.tex <==
0:43

==> assets/419-2/ReFoCUS/time11.tex <==
0:45

==> assets/419-2/ReFoCUS/time12.tex <==
0:49

==> assets/419-2/ReFoCUS/time13.tex <==
0:51

==> assets/419-2/ReFoCUS/time14.tex <==
0:52

==> assets/419-2/ReFoCUS/time15.tex <==
2:36

==> assets/419-2/ReFoCUS/time16.tex <==
4:44

==> assets/419-2/ReFoCUS/time17.tex <==
4:57

==> assets/419-2/ReFoCUS/time18.tex <==
5:03

==> assets/419-2/ReFoCUS/time19.tex <==
5:08

==> assets/419-2/ReFoCUS/time2.tex <==
0:08

==> assets/419-2/ReFoCUS/time20.tex <==
9:13

==> assets/419-2/ReFoCUS/time21.tex <==
9:17

==> assets/419-2/ReFoCUS/time22.tex <==
9:19

==> assets/419-2/ReFoCUS/time23.tex <==
9:29

==> assets/419-2/ReFoCUS/time24.tex <==
9:32

==> assets/419-2/ReFoCUS/time25.tex <==
9:33

==> assets/419-2/ReFoCUS/time26.tex <==
9:36

==> assets/419-2/ReFoCUS/time27.tex <==
10:07

==> assets/419-2/ReFoCUS/time28.tex <==
10:58

==> assets/419-2/ReFoCUS/time29.tex <==
11:01

==> assets/419-2/ReFoCUS/time3.tex <==
0:10

==> assets/419-2/ReFoCUS/time30.tex <==
11:12

==> assets/419-2/ReFoCUS/time31.tex <==
11:15

==> assets/419-2/ReFoCUS/time32.tex <==
11:39

==> assets/419-2/ReFoCUS/time4.tex <==
0:26

==> assets/419-2/ReFoCUS/time5.tex <==
0:27

==> assets/419-2/ReFoCUS/time6.tex <==
0:29

==> assets/419-2/ReFoCUS/time7.tex <==
0:30

==> assets/419-2/ReFoCUS/time8.tex <==
0:32

==> assets/419-2/ReFoCUS/time9.tex <==
0:33

==> assets/419-2/Uniform/response.tex <==
\WA{D. Middle of the video.}

==> assets/419-2/Uniform/time1.tex <==
0:00

==> assets/419-2/Uniform/time10.tex <==
3:36

==> assets/419-2/Uniform/time11.tex <==
4:00

==> assets/419-2/Uniform/time12.tex <==
4:24

==> assets/419-2/Uniform/time13.tex <==
4:48

==> assets/419-2/Uniform/time14.tex <==
5:12

==> assets/419-2/Uniform/time15.tex <==
5:36

==> assets/419-2/Uniform/time16.tex <==
6:00

==> assets/419-2/Uniform/time17.tex <==
6:25

==> assets/419-2/Uniform/time18.tex <==
6:49

==> assets/419-2/Uniform/time19.tex <==
7:13

==> assets/419-2/Uniform/time2.tex <==
0:24

==> assets/419-2/Uniform/time20.tex <==
7:37

==> assets/419-2/Uniform/time21.tex <==
8:01

==> assets/419-2/Uniform/time22.tex <==
8:25

==> assets/419-2/Uniform/time23.tex <==
8:49

==> assets/419-2/Uniform/time24.tex <==
9:13

==> assets/419-2/Uniform/time25.tex <==
9:37

==> assets/419-2/Uniform/time26.tex <==
10:01

==> assets/419-2/Uniform/time27.tex <==
10:25

==> assets/419-2/Uniform/time28.tex <==
10:49

==> assets/419-2/Uniform/time29.tex <==
11:13

==> assets/419-2/Uniform/time3.tex <==
0:48

==> assets/419-2/Uniform/time30.tex <==
11:37

==> assets/419-2/Uniform/time31.tex <==
12:01

==> assets/419-2/Uniform/time32.tex <==
12:25

==> assets/419-2/Uniform/time4.tex <==
1:12

==> assets/419-2/Uniform/time5.tex <==
1:36

==> assets/419-2/Uniform/time6.tex <==
2:00

==> assets/419-2/Uniform/time7.tex <==
2:24

==> assets/419-2/Uniform/time8.tex <==
2:48

==> assets/419-2/Uniform/time9.tex <==
3:12

==> assets/419-2/options.tex <==
\item A. There is no interview with a man in red clothing.
\item B. End of the video.
\item \ANS{C. Beginning of the video.}
\item D. Middle of the video.


==> assets/419-2/questions.tex <==
In which part of the video is a man wearing a red jersey interviewed?

==> assets/479-1/MDP3/response.tex <==
\WA{D. (b)(d)(a)(c).}

==> assets/479-1/MDP3/time1.tex <==
0:00

==> assets/479-1/MDP3/time10.tex <==
3:08

==> assets/479-1/MDP3/time11.tex <==
3:18

==> assets/479-1/MDP3/time12.tex <==
3:45

==> assets/479-1/MDP3/time13.tex <==
4:21

==> assets/479-1/MDP3/time14.tex <==
4:26

==> assets/479-1/MDP3/time15.tex <==
4:47

==> assets/479-1/MDP3/time16.tex <==
5:03

==> assets/479-1/MDP3/time17.tex <==
6:27

==> assets/479-1/MDP3/time18.tex <==
6:37

==> assets/479-1/MDP3/time19.tex <==
6:43

==> assets/479-1/MDP3/time2.tex <==
0:15

==> assets/479-1/MDP3/time20.tex <==
6:53

==> assets/479-1/MDP3/time21.tex <==
6:58

==> assets/479-1/MDP3/time22.tex <==
7:30

==> assets/479-1/MDP3/time23.tex <==
7:56

==> assets/479-1/MDP3/time24.tex <==
8:17

==> assets/479-1/MDP3/time25.tex <==
8:38

==> assets/479-1/MDP3/time26.tex <==
8:53

==> assets/479-1/MDP3/time27.tex <==
8:59

==> assets/479-1/MDP3/time28.tex <==
9:35

==> assets/479-1/MDP3/time29.tex <==
9:46

==> assets/479-1/MDP3/time3.tex <==
0:41

==> assets/479-1/MDP3/time30.tex <==
10:33

==> assets/479-1/MDP3/time31.tex <==
10:54

==> assets/479-1/MDP3/time32.tex <==
11:04

==> assets/479-1/MDP3/time4.tex <==
0:47

==> assets/479-1/MDP3/time5.tex <==
1:02

==> assets/479-1/MDP3/time6.tex <==
1:49

==> assets/479-1/MDP3/time7.tex <==
2:21

==> assets/479-1/MDP3/time8.tex <==
2:26

==> assets/479-1/MDP3/time9.tex <==
2:42

==> assets/479-1/ReFoCUS/response.tex <==
\ANS{B. (a)(c)(b)(d).}

==> assets/479-1/ReFoCUS/time1.tex <==
0:01

==> assets/479-1/ReFoCUS/time10.tex <==
0:16

==> assets/479-1/ReFoCUS/time11.tex <==
0:18

==> assets/479-1/ReFoCUS/time12.tex <==
0:19

==> assets/479-1/ReFoCUS/time13.tex <==
0:20

==> assets/479-1/ReFoCUS/time14.tex <==
0:22

==> assets/479-1/ReFoCUS/time15.tex <==
0:23

==> assets/479-1/ReFoCUS/time16.tex <==
0:24

==> assets/479-1/ReFoCUS/time17.tex <==
0:26

==> assets/479-1/ReFoCUS/time18.tex <==
0:27

==> assets/479-1/ReFoCUS/time19.tex <==
0:28

==> assets/479-1/ReFoCUS/time2.tex <==
0:03

==> assets/479-1/ReFoCUS/time20.tex <==
0:29

==> assets/479-1/ReFoCUS/time21.tex <==
0:36

==> assets/479-1/ReFoCUS/time22.tex <==
0:55

==> assets/479-1/ReFoCUS/time23.tex <==
4:43

==> assets/479-1/ReFoCUS/time24.tex <==
5:48

==> assets/479-1/ReFoCUS/time25.tex <==
7:00

==> assets/479-1/ReFoCUS/time26.tex <==
7:13

==> assets/479-1/ReFoCUS/time27.tex <==
7:17

==> assets/479-1/ReFoCUS/time28.tex <==
7:43

==> assets/479-1/ReFoCUS/time29.tex <==
8:13

==> assets/479-1/ReFoCUS/time3.tex <==
0:06

==> assets/479-1/ReFoCUS/time30.tex <==
8:20

==> assets/479-1/ReFoCUS/time31.tex <==
8:22

==> assets/479-1/ReFoCUS/time32.tex <==
8:23

==> assets/479-1/ReFoCUS/time4.tex <==
0:07

==> assets/479-1/ReFoCUS/time5.tex <==
0:09

==> assets/479-1/ReFoCUS/time6.tex <==
0:10

==> assets/479-1/ReFoCUS/time7.tex <==
0:11

==> assets/479-1/ReFoCUS/time8.tex <==
0:14

==> assets/479-1/ReFoCUS/time9.tex <==
0:15

==> assets/479-1/Uniform/response.tex <==
\WA{C. (b)(c)(d)(a).}

==> assets/479-1/Uniform/time1.tex <==
0:00

==> assets/479-1/Uniform/time10.tex <==
3:13

==> assets/479-1/Uniform/time11.tex <==
3:34

==> assets/479-1/Uniform/time12.tex <==
3:55

==> assets/479-1/Uniform/time13.tex <==
4:17

==> assets/479-1/Uniform/time14.tex <==
4:38

==> assets/479-1/Uniform/time15.tex <==
5:00

==> assets/479-1/Uniform/time16.tex <==
5:21

==> assets/479-1/Uniform/time17.tex <==
5:43

==> assets/479-1/Uniform/time18.tex <==
6:04

==> assets/479-1/Uniform/time19.tex <==
6:26

==> assets/479-1/Uniform/time2.tex <==
0:21

==> assets/479-1/Uniform/time20.tex <==
6:47

==> assets/479-1/Uniform/time21.tex <==
7:08

==> assets/479-1/Uniform/time22.tex <==
7:30

==> assets/479-1/Uniform/time23.tex <==
7:51

==> assets/479-1/Uniform/time24.tex <==
8:13

==> assets/479-1/Uniform/time25.tex <==
8:34

==> assets/479-1/Uniform/time26.tex <==
8:56

==> assets/479-1/Uniform/time27.tex <==
9:17

==> assets/479-1/Uniform/time28.tex <==
9:39

==> assets/479-1/Uniform/time29.tex <==
10:00

==> assets/479-1/Uniform/time3.tex <==
0:42

==> assets/479-1/Uniform/time30.tex <==
10:21

==> assets/479-1/Uniform/time31.tex <==
10:43

==> assets/479-1/Uniform/time32.tex <==
11:04

==> assets/479-1/Uniform/time4.tex <==
1:04

==> assets/479-1/Uniform/time5.tex <==
1:25

==> assets/479-1/Uniform/time6.tex <==
1:47

==> assets/479-1/Uniform/time7.tex <==
2:08

==> assets/479-1/Uniform/time8.tex <==
2:30

==> assets/479-1/Uniform/time9.tex <==
2:51

==> assets/479-1/options.tex <==
\item A. (a)(b)(c)(d).
\item \ANS{B. (a)(c)(b)(d).}
\item C. (b)(c)(d)(a).
\item D. (b)(d)(a)(c).


==> assets/479-1/questions.tex <==
In which order are the first four cars driven out of the garage in this video?
(a) The yellow car.
(b) The black car.
(c) The silver car.
(d) The white car.

==> assets/618-1/MDP3/response.tex <==
\WA{C. Du Fu’s route to Xi’an.}

==> assets/618-1/MDP3/time1.tex <==
0:27

==> assets/618-1/MDP3/time10.tex <==
16:15

==> assets/618-1/MDP3/time11.tex <==
19:30

==> assets/618-1/MDP3/time12.tex <==
19:58

==> assets/618-1/MDP3/time13.tex <==
20:26

==> assets/618-1/MDP3/time14.tex <==
22:17

==> assets/618-1/MDP3/time15.tex <==
26:00

==> assets/618-1/MDP3/time16.tex <==
27:24

==> assets/618-1/MDP3/time17.tex <==
28:48

==> assets/618-1/MDP3/time18.tex <==
31:35

==> assets/618-1/MDP3/time19.tex <==
32:31

==> assets/618-1/MDP3/time2.tex <==
1:51

==> assets/618-1/MDP3/time20.tex <==
35:18

==> assets/618-1/MDP3/time21.tex <==
38:33

==> assets/618-1/MDP3/time22.tex <==
39:29

==> assets/618-1/MDP3/time23.tex <==
39:57

==> assets/618-1/MDP3/time24.tex <==
41:48

==> assets/618-1/MDP3/time25.tex <==
42:44

==> assets/618-1/MDP3/time26.tex <==
47:23

==> assets/618-1/MDP3/time27.tex <==
47:51

==> assets/618-1/MDP3/time28.tex <==
48:18

==> assets/618-1/MDP3/time29.tex <==
50:10

==> assets/618-1/MDP3/time3.tex <==
2:19

==> assets/618-1/MDP3/time30.tex <==
52:57

==> assets/618-1/MDP3/time31.tex <==
56:40

==> assets/618-1/MDP3/time32.tex <==
58:32

==> assets/618-1/MDP3/time4.tex <==
5:34

==> assets/618-1/MDP3/time5.tex <==
6:30

==> assets/618-1/MDP3/time6.tex <==
7:25

==> assets/618-1/MDP3/time7.tex <==
11:36

==> assets/618-1/MDP3/time8.tex <==
12:04

==> assets/618-1/MDP3/time9.tex <==
13:28

==> assets/618-1/ReFoCUS/response.tex <==
\ANS{B. The Silk Road.}

==> assets/618-1/ReFoCUS/time1.tex <==
0:00

==> assets/618-1/ReFoCUS/time10.tex <==
1:36

==> assets/618-1/ReFoCUS/time11.tex <==
1:43

==> assets/618-1/ReFoCUS/time12.tex <==
1:50

==> assets/618-1/ReFoCUS/time13.tex <==
1:57

==> assets/618-1/ReFoCUS/time14.tex <==
2:04

==> assets/618-1/ReFoCUS/time15.tex <==
2:11

==> assets/618-1/ReFoCUS/time16.tex <==
2:18

==> assets/618-1/ReFoCUS/time17.tex <==
2:25

==> assets/618-1/ReFoCUS/time18.tex <==
3:00

==> assets/618-1/ReFoCUS/time19.tex <==
3:07

==> assets/618-1/ReFoCUS/time2.tex <==
0:13

==> assets/618-1/ReFoCUS/time20.tex <==
3:13

==> assets/618-1/ReFoCUS/time21.tex <==
3:48

==> assets/618-1/ReFoCUS/time22.tex <==
4:37

==> assets/618-1/ReFoCUS/time23.tex <==
4:44

==> assets/618-1/ReFoCUS/time24.tex <==
4:50

==> assets/618-1/ReFoCUS/time25.tex <==
4:57

==> assets/618-1/ReFoCUS/time26.tex <==
5:04

==> assets/618-1/ReFoCUS/time27.tex <==
5:11

==> assets/618-1/ReFoCUS/time28.tex <==
7:23

==> assets/618-1/ReFoCUS/time29.tex <==
8:11

==> assets/618-1/ReFoCUS/time3.tex <==
0:20

==> assets/618-1/ReFoCUS/time30.tex <==
10:23

==> assets/618-1/ReFoCUS/time31.tex <==
12:07

==> assets/618-1/ReFoCUS/time32.tex <==
31:38

==> assets/618-1/ReFoCUS/time4.tex <==
0:27

==> assets/618-1/ReFoCUS/time5.tex <==
0:34

==> assets/618-1/ReFoCUS/time6.tex <==
0:41

==> assets/618-1/ReFoCUS/time7.tex <==
0:48

==> assets/618-1/ReFoCUS/time8.tex <==
1:09

==> assets/618-1/ReFoCUS/time9.tex <==
1:16

==> assets/618-1/Uniform/response.tex <==
\WA{C. Du Fu’s route to Xi’an.}

==> assets/618-1/Uniform/time1.tex <==
0:00

==> assets/618-1/Uniform/time10.tex <==
17:07

==> assets/618-1/Uniform/time11.tex <==
19:01

==> assets/618-1/Uniform/time12.tex <==
20:56

==> assets/618-1/Uniform/time13.tex <==
22:50

==> assets/618-1/Uniform/time14.tex <==
24:44

==> assets/618-1/Uniform/time15.tex <==
26:38

==> assets/618-1/Uniform/time16.tex <==
28:32

==> assets/618-1/Uniform/time17.tex <==
30:27

==> assets/618-1/Uniform/time18.tex <==
32:21

==> assets/618-1/Uniform/time19.tex <==
34:15

==> assets/618-1/Uniform/time2.tex <==
1:54

==> assets/618-1/Uniform/time20.tex <==
36:09

==> assets/618-1/Uniform/time21.tex <==
38:03

==> assets/618-1/Uniform/time22.tex <==
39:58

==> assets/618-1/Uniform/time23.tex <==
41:52

==> assets/618-1/Uniform/time24.tex <==
43:46

==> assets/618-1/Uniform/time25.tex <==
45:40

==> assets/618-1/Uniform/time26.tex <==
47:34

==> assets/618-1/Uniform/time27.tex <==
49:29

==> assets/618-1/Uniform/time28.tex <==
51:23

==> assets/618-1/Uniform/time29.tex <==
53:17

==> assets/618-1/Uniform/time3.tex <==
3:48

==> assets/618-1/Uniform/time30.tex <==
55:11

==> assets/618-1/Uniform/time31.tex <==
57:05

==> assets/618-1/Uniform/time32.tex <==
59:00

==> assets/618-1/Uniform/time4.tex <==
5:42

==> assets/618-1/Uniform/time5.tex <==
7:36

==> assets/618-1/Uniform/time6.tex <==
9:30

==> assets/618-1/Uniform/time7.tex <==
11:25

==> assets/618-1/Uniform/time8.tex <==
13:19

==> assets/618-1/Uniform/time9.tex <==
15:13

==> assets/618-1/options.tex <==
\item A. The Yellow River.
\item \ANS{B. The Silk Road.}
\item C. Du Fu's route to Xi'an.
\item D. The Yangtze River.


==> assets/618-1/questions.tex <==
What do the expanding red lines on the map in the first few minutes of the video stand for?

==> assets/792-1/MDP3/response.tex <==
\WA{B. 9.}

==> assets/792-1/MDP3/time1.tex <==
0:16

==> assets/792-1/MDP3/time10.tex <==
8:49

==> assets/792-1/MDP3/time11.tex <==
9:21

==> assets/792-1/MDP3/time12.tex <==
10:41

==> assets/792-1/MDP3/time13.tex <==
10:57

==> assets/792-1/MDP3/time14.tex <==
12:18

==> assets/792-1/MDP3/time15.tex <==
15:14

==> assets/792-1/MDP3/time16.tex <==
15:46

==> assets/792-1/MDP3/time17.tex <==
16:18

==> assets/792-1/MDP3/time18.tex <==
16:50

==> assets/792-1/MDP3/time19.tex <==
17:39

==> assets/792-1/MDP3/time2.tex <==
0:32

==> assets/792-1/MDP3/time20.tex <==
18:43

==> assets/792-1/MDP3/time21.tex <==
19:15

==> assets/792-1/MDP3/time22.tex <==
20:19

==> assets/792-1/MDP3/time23.tex <==
20:51

==> assets/792-1/MDP3/time24.tex <==
21:07

==> assets/792-1/MDP3/time25.tex <==
23:16

==> assets/792-1/MDP3/time26.tex <==
23:48

==> assets/792-1/MDP3/time27.tex <==
25:08

==> assets/792-1/MDP3/time28.tex <==
26:44

==> assets/792-1/MDP3/time29.tex <==
27:32

==> assets/792-1/MDP3/time3.tex <==
2:40

==> assets/792-1/MDP3/time30.tex <==
28:37

==> assets/792-1/MDP3/time31.tex <==
29:09

==> assets/792-1/MDP3/time32.tex <==
30:45

==> assets/792-1/MDP3/time4.tex <==
4:00

==> assets/792-1/MDP3/time5.tex <==
4:48

==> assets/792-1/MDP3/time6.tex <==
5:20

==> assets/792-1/MDP3/time7.tex <==
6:57

==> assets/792-1/MDP3/time8.tex <==
7:29

==> assets/792-1/MDP3/time9.tex <==
8:33

==> assets/792-1/ReFoCUS/response.tex <==
\WA{D. 7.}

==> assets/792-1/ReFoCUS/time1.tex <==
0:11

==> assets/792-1/ReFoCUS/time10.tex <==
2:39

==> assets/792-1/ReFoCUS/time11.tex <==
2:59

==> assets/792-1/ReFoCUS/time12.tex <==
3:11

==> assets/792-1/ReFoCUS/time13.tex <==
3:19

==> assets/792-1/ReFoCUS/time14.tex <==
3:55

==> assets/792-1/ReFoCUS/time15.tex <==
3:59

==> assets/792-1/ReFoCUS/time16.tex <==
4:03

==> assets/792-1/ReFoCUS/time17.tex <==
4:07

==> assets/792-1/ReFoCUS/time18.tex <==
4:11

==> assets/792-1/ReFoCUS/time19.tex <==
4:43

==> assets/792-1/ReFoCUS/time2.tex <==
1:03

==> assets/792-1/ReFoCUS/time20.tex <==
4:47

==> assets/792-1/ReFoCUS/time21.tex <==
4:51

==> assets/792-1/ReFoCUS/time22.tex <==
4:55

==> assets/792-1/ReFoCUS/time23.tex <==
5:23

==> assets/792-1/ReFoCUS/time24.tex <==
5:38

==> assets/792-1/ReFoCUS/time25.tex <==
5:46

==> assets/792-1/ReFoCUS/time26.tex <==
5:58

==> assets/792-1/ReFoCUS/time27.tex <==
6:14

==> assets/792-1/ReFoCUS/time28.tex <==
6:18

==> assets/792-1/ReFoCUS/time29.tex <==
7:42

==> assets/792-1/ReFoCUS/time3.tex <==
1:15

==> assets/792-1/ReFoCUS/time30.tex <==
8:34

==> assets/792-1/ReFoCUS/time31.tex <==
9:10

==> assets/792-1/ReFoCUS/time32.tex <==
11:49

==> assets/792-1/ReFoCUS/time4.tex <==
1:47

==> assets/792-1/ReFoCUS/time5.tex <==
1:59

==> assets/792-1/ReFoCUS/time6.tex <==
2:03

==> assets/792-1/ReFoCUS/time7.tex <==
2:07

==> assets/792-1/ReFoCUS/time8.tex <==
2:11

==> assets/792-1/ReFoCUS/time9.tex <==
2:19

==> assets/792-1/Uniform/response.tex <==
\WA{C. 8.}

==> assets/792-1/Uniform/time1.tex <==
0:00

==> assets/792-1/Uniform/time10.tex <==
9:51

==> assets/792-1/Uniform/time11.tex <==
10:57

==> assets/792-1/Uniform/time12.tex <==
12:03

==> assets/792-1/Uniform/time13.tex <==
13:08

==> assets/792-1/Uniform/time14.tex <==
14:14

==> assets/792-1/Uniform/time15.tex <==
15:20

==> assets/792-1/Uniform/time16.tex <==
16:26

==> assets/792-1/Uniform/time17.tex <==
17:31

==> assets/792-1/Uniform/time18.tex <==
18:37

==> assets/792-1/Uniform/time19.tex <==
19:43

==> assets/792-1/Uniform/time2.tex <==
1:05

==> assets/792-1/Uniform/time20.tex <==
20:49

==> assets/792-1/Uniform/time21.tex <==
21:54

==> assets/792-1/Uniform/time22.tex <==
23:00

==> assets/792-1/Uniform/time23.tex <==
24:06

==> assets/792-1/Uniform/time24.tex <==
25:12

==> assets/792-1/Uniform/time25.tex <==
26:17

==> assets/792-1/Uniform/time26.tex <==
27:23

==> assets/792-1/Uniform/time27.tex <==
28:29

==> assets/792-1/Uniform/time28.tex <==
29:34

==> assets/792-1/Uniform/time29.tex <==
30:40

==> assets/792-1/Uniform/time3.tex <==
2:11

==> assets/792-1/Uniform/time30.tex <==
31:46

==> assets/792-1/Uniform/time31.tex <==
32:52

==> assets/792-1/Uniform/time32.tex <==
33:57

==> assets/792-1/Uniform/time4.tex <==
3:17

==> assets/792-1/Uniform/time5.tex <==
4:22

==> assets/792-1/Uniform/time6.tex <==
5:28

==> assets/792-1/Uniform/time7.tex <==
6:34

==> assets/792-1/Uniform/time8.tex <==
7:40

==> assets/792-1/Uniform/time9.tex <==
8:45

==> assets/792-1/options.tex <==
\item \ANS{A. 10.}
\item B. 9.
\item C. 8.
\item D. 7.


==> assets/792-1/questions.tex <==
How many magic shows are included in this video?
